Ensembling Strategies for Answering Natural Questions

Many of the top question answering systems today utilize ensembling to improve their performance on tasks such as the Stanford Question Answering Dataset (SQuAD) and Natural Questions (NQ) challenges. Unfortunately most of these systems do not publish their ensembling strategies used in their leaderboard submissions. In this work, we investigate a number of ensembling techniques and demonstrate a strategy which improves our F1 score for short answers on the dev set for NQ by 2.3 F1 points over our single model (which outperforms the previous SOTA by 1.9 F1 points).

==> experiments.bak.0.tex <==
\section{Experiments}
% Table showcasing experimental results on "train/test" split
We examine two types of ensembling experiments: (i) ensembling the same model trained with different seeds and (ii) ensembling different models.  Ensembling the same model trained on different seeds attempts to smooth the variance to produce a stronger result.  On the other hand ensembling different models attempts to find models that may not be the strongest individually but harmonize well to produce strong results.
Throughout this section we will use \saDevTrain, \laDevTrain, \saDevTest, \laDevTest to denote the short and long answer performance on dev train and test.  Similarly we will use \numModelsSearched to indicate the number of models searched for an experiment and \numModels to indicate the number of models an experiment uses to optimize short and long answer F1 performance.

%Throughout this section we will use SA F1\footnote{SA F1 score on dev-train data.\label{fn:sa-train}}, LA F1\footnote{LA F1 score on dev-train data.\label{fn:la-train}}, SA F1\footnote{SA F1 score on dev-test data.\label{fn:sa-test}}, LA F1\footnote{LA F1 score on dev-test data.\label{fn:la-test}} to denote the short and long answer performance on dev train and test.

\subsection{Seed experiments}
% Showing relative ineffectiveness of ensembling the same model with diff seeds


We select the single model with the highest sum of short and long answer F1 scores and train it with $k$ different seeds.  % necessary to repeat??
In table \ref{tab:exp:seed} we find that there is a benefit to ensembling multiple versions of the same model trained with different seeds\footnote{Note that there is some data snooping ocuring here as models are selected based on full dev performance (which is a superset of ``dev-test'').}.

\avi{pls center all the tables and add a hline to them. I added to the one below..}

\begin{table}[]
\small
\centering
\begin{tabular}{lll}
\toprule %\hline
\# Models  & \saDevTest & \laDevTest   \\
\toprule %\hline
1  & 0.5614 & 0.6710  \\
\hline
4  & \textbf{0.5873} & \textbf{0.6961} \\
\bottomrule %\hline
\end{tabular}
\caption{Ensembling the same model trained with different seeds.}
\label{tab:exp:seed}
\end{table}

\subsection{Main experiments}
% Table of experiments
% Experiments that I can include:
% Basic Greedy: 5
% Basic Exhaustive: 2
% Basic Greedy on candidates from Basic Exhaustive: 5 (probably just mention single summary sentence for these to save space)
% Take top-k performing LA or SA on dev (snooping): 2
% Greedy Sum: 5

% Normalized:
% Greedy Linearly Decaying Sum: 5
% Greedy Exponentially Decaying Sum: 5
% Greedy Noisy Or: 5

% Follow up expts: 3

% Notes:
% - Almost all of the normalized expts use logistic regression that is snooping.  Ran 2 experiments with one that doesn't to confirm no impact of snooping
% - Ran some informal expts (on candidates submitted to leaderboard last time) which showed that the aggregation expts needed normalization too.  Thinking I just mention that results for these are ommitted for brevity since they do not show anything interesting (other than that collectively they are poor results)
% Maybe after basic expts just show optimizing for LA since that generalizes best
% Columns: [Row, Search Strategy, Normalization Strategy, Aggregation Strategy, Num models searched, Num Models, Num SA models, Num LA models, SA F1 Search, LA F1 Search, F1 F1 Eval, LA F1 Eval]

% Table \anthony{TODO: ref} shows several experiments with different search, normalization, and aggregation strategies.  We also investigated the IR aggregation approaches without normalization, however we omit these results here for brevity as they did not perform nearly as well as when normalization was applied.

% - Greedy vs Exhaustive vs Simple Greedy [Search Strategy, Num models searched, Num SA models, Num LA models, SA F1 Search, LA F1 Search, F1 F1 Eval, LA F1 Eval]
%     - Conclusion: Use greedy and all optimize for LA since they generalize better

\begin{table*}[]
\small
\centering
\begin{tabular}{llllllll}
\toprule
 Search & \numModelsSearched & \numModels  & \saDevTrain & \laDevTrain & \saDevTest & \laDevTest   \\
 \toprule
 %Simple Greedy & 4 & 0/4 & N/A & N/A & 0.5925 & 0.6902  \\
 %Simple Greedy & 4 & 4/0 & N/A & N/A & 0.5762 & 0.6816   \\
 ES & 20 & 0/4 & 0.5922 & \textbf{0.6989} & 0.5964 & 0.7049   \\
 \hline
 ES & 20 & 4/0 & \textbf{0.5925} & 0.6902 & 0.5964 & 0.6998   \\
 \hline
 GS & 41 & 0/4 & 0.5857 & 0.6972 & \textbf{0.5971} & 0.7084  \\
 \hline
 GS & 41 & 1/3 & 0.5767 & 0.6929 & 0.5863 & 0.\textbf{7097}    \\
 \hline
 GS & 41 & 2/2 & 0.5837 & 0.6932 & 0.5864 & 0.7089    \\
 \hline
 GS & 41 & 3/1 & 0.5883 & 0.6853 & 0.5857 & 0.7060    \\
 \hline
 GS & 41 & 4/0 & 0.5897 & 0.6922 & 0.5907 & 0.6981   \\
 \bottomrule
\end{tabular}
%\avi{abbreviate column names. may even remove first 2 rows. add hlines}
\caption{Comparison of Search Strategies.  All experiments run without normalization using the max aggregator.}
\label{tab:exp:ens:search}
\end{table*}

We investigate the different search strategies in table \ref{tab:exp:ens:search}.  We see that the simple greedy approach is not as good as either the exhaustive or greedy approaches\footnote{Note that the models were selected based on dev set performance rather than ``dev-train`` performance yielding optimistic eval scores, however they are still lower than for the other approaches.} and further note that the simple greedy ensemble optimized for long answers outperforms the one optimized for short answers on both short and long answers on the ``dev-test'' set.  For the exhaustive approach we see that it obtains the best long and short F1 scores on ``dev-train'' for the respective models as expected, however these do not translate to the best scores on ``dev-test''.  We find that the greedy approach performs best overall, with the greedy ensemble optimized exclusively for long answer performance performing the best on short answer F1 and is 0.0013 F1 lower than the best long answer F1 on ``dev-test''.  Also note that the numbers seen here, praticularly when optimizing greedily ofr long answer performance are higher than those observed for ensembling the same model with multiple seeds in table \ref{tab:exp:seed}.

We hypothesize \anthony{TODO better word?} that the reasons for the superior generalization of the greedy approach over exhaustive is that exhaustive search is ``overfitting''.  Another potential cause of the better generalization of greedy is that it can search more candidates.  Whereas with the greedy approach we can search all 41 candidates\footnote{candidate models represent models trained with different model types (e.g. BERT for QA and AoA) and hyperparameters (e.g. learning rate and negative example subsampling rate)}, with exhaustive search we only consider our top 20 (by sum of short and long answer F1) for runtime considerations.  This gives the greedy strategy a more diverse set of candidates to work with.  Similarly we hypothesize the reason optimizing for long answer F1 generalizes better for short and long answers is due to the strict definition of correctness for Natural Questions which requires exact span matching \cite{Kwiatkowski2019NaturalQA}.  For the remainder of this paper we will focus on greedy search with all four models optimized for long answer to keep the number of experiments presented to a manageable level.  Note that further experimentation with different short and long answer optimization trade-offs confirm the conclusion here that optimizing for long answer performance generalizes the best.

% - Greedy with all candidates vs candidates chosen from exhaustive [Num models searched, Num SA models, Num LA models, SA F1 Search, LA F1 Search, F1 F1 Eval, LA F1 Eval]
%     - Conclusion: There is some benefit to using all candidates (and it’s quick enough with greedy) to use all

\begin{table}[]
\small
\centering
\begin{tabular}{lllll}
\toprule
\numModelsSearched  & \saDevTrain & \laDevTrain & \saDevTest & \laDevTest   \\
\toprule
41  & 0.5857 & \textbf{0.6972} & \textbf{0.5971} & \textbf{0.7084}  \\
\hline
20  & \textbf{0.5860} & 0.6951 & 0.5896 & 0.704    \\
\bottomrule
\end{tabular}
\caption{Impact of candidate pool size.  All experiments run with a greedy search strategy optimized exlcusively for long answer F1 without normalization using the max aggregator.}
\label{tab:exp:ens:candidates}
\end{table}

In table \ref{tab:exp:ens:candidates} we investigate the impact of the candidate model search space size.  We use the greedy search strategy to optimize for long answer performance without normalization using the max aggregator.  For the experiment with 20 candidates we use the same 20 candidates as for the exhaustive search strategy experiment (greatest sum of short and long answer F1s).  We find that the added diversity of the models avaible in the entire pool produces a stronger ensemble which generalizes better both in short and long answer F1.  Having verified the benefit of using the entire candidate pool we continue to do so in the remainder of our experiments.


% - Greedy Sum [Num SA models, Num LA models, SA F1 Search, LA F1 Search, F1 F1 Eval, LA F1 Eval]
%     - Conclusion: sum is worse than max
%     - Would like to do something better than make a table just for this but noting immediately comes to mind
%     - I also have exhaustive sum if we think it would be good to add that
%     - I’m assuming when we cut this will be one of the first tables to go

% \begin{table}[]
% \small
% \begin{tabular}{lllll}
% Strat.  & \saDevTrain & \laDevTrain & \saDevTest & \laDevTest   \\
% Max  & \textbf{0.5857} & \textbf{0.6972} & \textbf{0.5971} & \textbf{0.7084}  \\
% Sum  & 0.4382 & 0.6873 & TODO & TODO    
% \end{tabular}
% %\avi{sometimes you can put the column names on top of each other by using an extra line. Can't tiny anything. }
% \caption{Comparison of max and sum aggregation strategies.  All experiments run with a greedy search strategy optimized exclusively for long answer F1 without normalization.}
% \label{tab:exp:ens:sum}
% \end{table}

% We compare the results of the sum and max aggregators in table \ref{tab:exp:ens:sum}.  All experiments are run with the greedy search strategy over the full pool of 41 candidates without normalization. \anthony{TODO: run eval numbers for sum and add results to table and here}


% - Greedy Normalized with different aggregation types [Aggregation strategy, Num SA models, Num LA models, SA F1 Search, LA F1 Search, F1 F1 Eval, LA F1 Eval]
%     - Conclusion: Noisy Or helps LA, all approaches hurt SA

\begin{table}[]
\small
\centering
\begin{tabular}{lllll}
\toprule
Agg.  & \saDevTrain & \laDevTrain & \saDevTest & \laDevTest   \\
\toprule
Max  & \textbf{0.5857} & 0.6972 & \textbf{0.5971} & 0.7084  \\
\hline
ExS  & 0.5619 & 0.6944 & 0.5826 & 0.7040  \\
\hline
RRS  & 0.5553 & 0.6954 & 0.5728 & 0.7066  \\
\hline
NO  & 0.5545 & \textbf{0.7037} & 0.573 & \textbf{0.715}  \\
\bottomrule
\end{tabular}
\caption{Comparison of IR inspired aggregation strategies (A.).  All experiments run with a greedy search strategy optimized exclusively for long answer F1 with logistic regression normalization (except max which is not normalized).}
\label{tab:exp:ens:norm-agg}
\end{table}

We investigate the impact of the IR inspired normalization strategies in table \ref{tab:exp:ens:norm-agg}.  The max experiment is as-before run without normalization to greedily optimize for long answer F1.  The other experiments here are normalization with logistic regression, as our experiments showed that not normalizing decreased performance.  We find that using max aggregation results in the best short answer F1 whereas using normalized noisy or aggregation results in the best long answer F1.


% - I also have a couple follow up experiments which I would like to put in a table, but the descriptions of them would be a little much to put in a table
%     - Conclusion: Use Noisy or (normalized) on LA and max (unnormalized) on SA.  Also, selecting candidates by using Greedy then doing noisy or for LA and max for SA may help both LA and SA performance (+~0.3-0.4 each F1 on ~3200 examples)

\anthony{TODO: update below table with new expt numbers}

\begin{table}[]
\small
\centering
\begin{tabular}{lll}
\toprule
MSAS  & \saDevTest & \laDevTest   \\
\toprule
Max  & \textbf{0.5971} & \textbf{0.7179} \\
\hline
NO  & 0.5934 & 0.7150 \\
\bottomrule
\end{tabular}
\caption{Experiments predicting using max for short answers and noisy or for long answers with models selected using aggregation strategy (MSAS) as shown in table.}
\label{tab:exp:combine}
\end{table}

% For these experiments the ensembled models are those selected from the max and noisy or experiments respectively in table \ref{tab:exp:ens:norm-agg}.

\anthony{TODO: Probably revise to clarify meaning of expt}

Based on our conclusions from table \ref{tab:exp:ens:norm-agg} that unnormalized max works best for short answers and logistic regression normalized noisy or works best for long answers we experiment with this configuration in table \ref{tab:exp:combine}.  We find that this approach produces the strongest performance for both short and long answers.  Further, we investigate selecting models using unnormalized max for both short and long answers, and then running with logistic regression normalized noisy or on the ``dev-test'' set.  This allows for a quicker ensemble model selection as logisitc regression does not need to be repeatedly run in the search phase.  We find that this approach does not decrease short answer or long answer F1 performance \anthony{TODO: significance to claim increases???}.  


\begin{table}[]
\small
\centering
\begin{tabular}{ll}
\toprule
Short Answer Containing Span  & \saDevTest    \\
\toprule
Any non-null  & \textbf{0.5971}  \\
\hline
Best long span  & 0.5836  \\
\bottomrule
\end{tabular}
\caption{Investigation of requiring short span predictions to be contained within the predicted long span.}
\label{tab:exp:restrict-sa-to-la}
\end{table}

\anthony{TODO: update these numbers as well after running expts with no snoop normalizer.  Probably revise to clarify meaning of expt}

To further improve short answer performance, we investigate the effectiveness of extending the approach from \ref{tab:exp:combine} by changing the core strategy so that short answers are required to be contained in the best long answer.  This follows from a requirement of \cite{Kwiatkowski2019NaturalQA} that short answers be contained in the long answer (if there is a short answer).  Surprisingly we find in table \ref{tab:exp:restrict-sa-to-la} that this decreases short answer performance.  We hypothesize that this is a result of incorrect long answer predictions forcing the system to predict an incorrect short answer, but leave a more formal examination to future work.


% In conclusion, we recommend using unnormalized max for short answers and logistic regression normalized noisy or for long answers when running an ensemble with models selected using unnormalized max for both short and long answer (for quicker model selection).

\anthony{TODO: final dev numbers for best approach}
